A Fast and Flexible Algorithm for the Graph-Fused Lasso

We propose a new algorithm for solving the graph-fused lasso (GFL), a method for parameter estimation that operates under the assumption that the signal tends to be locally constant over a predefined graph structure. Our key insight is to decompose the graph into a set of trails which can then each be solved efficiently using techniques for the ordinary (1D) fused lasso. We leverage these trails in a proximal algorithm that alternates between closed form primal updates and fast dual trail updates. The resulting techinque is both faster than previous GFL methods and more flexible in the choice of loss function and graph structure. Furthermore, we present two algorithms for constructing trail sets and show empirically that they offer a tradeoff between preprocessing time and convergence rate.

==> acceleration.tex <==

\section{Acceleration via locally adaptive penalties}
\label{sec:acceleration}
As we have seen in Section \ref{sec:grid_example}, the graph decomposition can have a substantial effect on the performance of the baseline ADMM algorithm. In that simple grid graph example, decomposing the graph along the rows and columns of the grid results in rapid convergence relative to the other trail sets. To better understand this effect, consider the squared loss update in \eqref{eqn:admm_updates_beta_squared_loss}. Note that each dual variable $z_j$ is weighted equally, that is, each is multiplied by the scalar penalty parameter $\alpha$. This effectively implies that each trail update equally informs how to update $\beta$, which seems unlikely given the fused aspect of the trail updates. A dual variable in a trail update is leveraging the information propagated by its ancestors and decendents, implemented in the form of the forward and backward updates in the dynamic programming solution we employ \citep{johnson:2013}. It is therefore reasonable to expect that dual variables in longer trails carry more information to the $\beta$ update than their shorter trail counterparts.

Balancing these primal update weights may then lead to more rapid convergence in the overall algorithm. Rather than using a scalar $\alpha$, we could instead use a symmetric positive definite matrix $P$ \citep{boyd:etal:2011} that places higher weight on longer trails. A line of recent work \citep{nishihara:etal:2015,fougner:etal:2015} has investigated determining optimal $\alpha$ choices for ADMM algorithms when $\alpha$ is a scalar. While it may be possible to extend these techniques to determine an optimal $P$ for a given set of trails, such an undertaking is outside of the scope of this paper. We instead propose a fast acceleration heuristic that attempts to improve (crudely) the balance of the updates.

Let $\mathcal{T} = \{ t_1, t_2, \ldots, t_k \}$ be a set of trails yielding $d$ slack variables in \eqref{eqn:trail_loss_function_duals}. $P = \text{diag}(\boldsymbol\rho)$ is a $d\times d$ diagonal matrix with diagonal values $\{ \boldsymbol\rho \in \real^d : \rho_j > 0, j = 1, 2, \ldots, d \}$. For a given scalar penalty $\alpha$,

\begin{equation}
\label{eqn:acceleration_diagonal}
\rho_j = [\frac{c k}{d}T(j) + (1 - c)]\alpha \, ,
\end{equation}

where $c \in [0, 1]$ is a hyperparameter and $T(j)$ is the length of the trail to which $z_j$ belongs. The first half term in the heuristic adjusts the $\alpha$ penalty on a per-trail basis, setting the penalty for each slack variable to be proportional to the length of its trail relative to the mean trail length. Since the heuristic is a rough approximation, the $c$ hyperparameter is used to dampen this heuristic, with $c=0$ recovering the original ADMM algorithm.

Figure \ref{fig:grid_example_c_test} shows the performance of the algorithm as $c$ changes. In the rows and columns decomposition, the heuristic has no effect since every trail in the square grid is exactly the length of the mean trail. At the extreme of $c=1$, using only the first term in the penalty equation, actually hinders convergence for the other two trails relative to their unaccelerated performance, suggesting that it is not perfectly capturing the underlying optimal penalty values. However, it does appear to help speed up convergence when the adjustment is dampened, making the balanced pseudo-trails as efficient as the unbalanced median trails for values in the range $[0.3,0.7]$. In other simulations we have found that values in the range $[0.2, 0.8]$ typically work well; for simplicity, we use $c=0.5$ for all of our subsequent experiments.

% \begin{figure}[tb]
%   \centering
%   \includegraphics[width=0.8\textwidth]{../../plots/trail_length_weight.pdf}
%   \caption{Performance of the accelerated algorithm as the damping hyperparameter $c$ is adjusted. For values around $c=0.5$, the pseudo-tour trails converge as quickly as the median trails.}
%   \label{fig:grid_example_c_test}
% \end{figure}


The resulting $\beta$ updates are then more balanced in terms of the weight given to each $z_j$. In the case of a squared loss, the update now becomes a non-uniformly weighted sum,

\begin{equation}
\label{eqn:admm_updates_beta_squared_loss_accelerated}
\beta_i^{k+1} = \frac{2y_i + \sum_{j \in \mathcal{J}} \rho_j (z_j - u_j)}{2 + \sum_{j \in \mathcal{J}} \rho_j} \, .
\end{equation}

Additionally, a straightforward adjustment must be made to $w$ in \eqref{eqn:admm_updates_z} to account for the varying penalty term.


